Temperature gradient driven heat flux closure in fluid simulations of collisionless reconnection

Recent efforts to include kinetic effects in fluid simulations of plasmas have been very promising. Concerning collisionless magnetic reconnection, it has been found before that damping of the pressure tensor to isotropy leads to good agreement with kinetic runs in certain scenarios. An accurate representation of kinetic effects in reconnection was achieved in a study by Wang et al. (Phys. Plasmas, volume 22, 2015, 012108) with a closure derived from earlier work by Hammett and Perkins (PRL, volume 64, 1990, 3019). Here, their approach is analyzed on the basis of heat flux data from a Vlasov simulation. As a result, we propose a new local closure in which heat flux is driven by temperature gradients. That way, a more realistic approximation of Landau damping in the collisionless regime is achieved. Previous issues are addressed and the agreement with kinetic simulations in different reconnection setups is improved significantly. To the authors' knowledge, the new fluid model is the first to perform well in simulations of the coalescence of large magnetic islands.

==> packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage[a4paper, top=3.5cm, bottom=4cm, inner=4.5cm, outer=3.5cm]{geometry}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{textcomp}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage[german,english]{babel}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{verbatim} % multi-line comments
\usepackage{gensymb}
\usepackage{ulem} % double underline
\usepackage[backend=bibtex,natbib=true,sorting=none]{biblatex}

